Evaluating and Improving Graph-based Explanation Methods for Multi-Agent Coordination

Graph Neural Networks (GNNs), developed by the graph learning community, have been adopted and shown to be highly effective in multi-robot and multi-agent learning. Inspired by this successful cross-pollination, we investigate and characterize the suitability of existing GNN explanation methods for explaining multi-agent coordination. We find that these methods have the potential to identify the most-influential communication channels that impact the team's behavior. Informed by our initial analyses, we propose an attention entropy regularization term that renders GAT-based policies more amenable to existing graph-based explainers. Intuitively, minimizing attention entropy incentivizes agents to limit their attention to the most influential or impactful agents, thereby easing the challenge faced by the explainer. We theoretically ground this intuition by showing that minimizing attention entropy increases the disparity between the explainer-generated subgraph and its complement. Evaluations across three tasks and three team sizes i) provides insights into the effectiveness of existing explainers, and ii) demonstrates that our proposed regularization consistently improves explanation quality without sacrificing task performance.

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/4_agent_zero_shot_from_3_policy/attn_ent/model/data/3 <==
¬‡¿HW¿uÌ<¿×WÇ>ED?ȧv¿M;ÀfŒ1¿Ô)¿/ÄE?7s"¿ö;?0?\‰×¿|*R¿&J£¿÷Ç?¹2»¿ô<î>G®¿ùi†>Ôý?CgÀ;¿Ji(À󕉿´ˆ¾¨qµ>øº¶¿×þÀj¯¿¸¯¿

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/4_agent_zero_shot_from_3_policy/no_attn_ent/model/data/0 <==
Xºå<ké´;bÜ<!ž»L+A¼7ÿ<Ù¸á<w^N:¨/ó;ŠA¼W\<0T;<|*»úѹ;—껧Ú3»~æq:*³<ࡗ»±(2½€ËÙ;]n#¼-(Ÿ:F±X¼Ž
½7æ"<¬•ãº¯'¼'=¯<¼–Š<,÷Ö;´

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/5_agent_zero_shot_from_3_policy/attn_ent/model/data/3 <==
¬‡¿HW¿uÌ<¿×WÇ>ED?ȧv¿M;ÀfŒ1¿Ô)¿/ÄE?7s"¿ö;?0?\‰×¿|*R¿&J£¿÷Ç?¹2»¿ô<î>G®¿ùi†>Ôý?CgÀ;¿Ji(À󕉿´ˆ¾¨qµ>øº¶¿×þÀj¯¿¸¯¿

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/5_agent_zero_shot_from_3_policy/no_attn_ent/model/data/0 <==
Xºå<ké´;bÜ<!ž»L+A¼7ÿ<Ù¸á<w^N:¨/ó;ŠA¼W\<0T;<|*»úѹ;—껧Ú3»~æq:*³<ࡗ»±(2½€ËÙ;]n#¼-(Ÿ:F±X¼Ž
½7æ"<¬•ãº¯'¼'=¯<¼–Š<,÷Ö;´

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/5_agent_zero_shot_from_4_policy/attn_ent/model/data/3 <==
ðß½÷>M#À°ŠV>"¿ÎMÚ>.áq¿²/ï¿÷bH¾Ä4Àäü¿we_¿¸%¿=Æ¾ìb¿½ÓÐ>ï-"¿êlÀ#ñ'¾)õe?Ӟ-¿¿­(ÀÐژ¿áGê>²׾)Ö?5m"=OïV¿×©´>\ô>£¹>BÌ?

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/5_agent_zero_shot_from_4_policy/no_attn_ent/model/data/1 <==
'Ç8½2D¾¾ã(¾ª"Ÿ>Žº½@
–>Ivp¿^‰¼>'•Ë¾5rY½	¤¿!Ñ&½±a?´8\?ª×>Àä¬>Z>çK9>Ouu?|‹â¾ã¥œ>N¡|½µ>Ðoœ=1f‡>³V?q¼q>룰>‰ê'=æ`>†p¤?ø7=¾×¹½,gï>%kô>2,Ÿ=ä9E¿|"¾Ñ>
¾ó}½†R?>ô'‹>Qu¾Ÿš¿Íu>¿äþ¾ÃŒ,:Àº}>ÞÀÿ=;n=Éíe>‰ÛľoJ¾eÚw¾ÿ¢¿ÕaX>‰†¾°œ=ϏX=;Y½Îо§.?Ž3¾}NË>w+¾ë%C>IÐ=ty8?Ð =6@A?-Ö3½7$¾˜:?¬ßí>²gŒ¾ö >ë}¬¾ʱ½©œ'¾\y•=N$Ð>邿>Kgø>ë'Ï>P㌽Çôe¿ÂkÅ>â–ľ!§>ub>[Y¿‰1>¯âö>Ä4i?ÜÝ>;8¾œH¿O£>
¸¾Íjœ=Š×<ƒ>¢›?Cʅ¾°æê=¾‹>‰:?Xà ½€Ï(>Ñ¿¾n	>ÿî§=Ç(5=u¡7¿ûj¼¾…r¿Z¨=ôÍ>ʵ¾hÏݾãŸÕ>4ö›½Ú>?V¼€­(>pB¢<}yO¿B0b¿ƒËö¾ˆ6¿•Cà<P=ø°¶½A©s?*<s½²–>Ć>0c½J"оÕz'>
ŒÓ>"ÿÊ>¸Ã…¾wG<?…j>CS?Ã>m/U¾ç2O?®q¾Ë:?o9Ã>×bÀ>c8€¿äÒ?_oÔ=kó[¾…3"?îm>Ò´Ç=÷ò¾ð"ª¾Ê™è;´Ê¿ú9¾Úo
¾9\
¿"W
?Jü`?z=¿>e=@]¾Ï뫽+¬©=ðð¾'%?_Èo¾	oˆ>Rk/½$À7?¡ìE<"èƒ?^…¾Â•<Q n>ÄÇ«>,ñI½Úî¾Í]Pb¾ ´ˆ>4v¡»

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/5_agent_zero_shot_from_4_policy/no_attn_ent/model/data/2 <==
ej¾É\#¼1"˾6ͼ1>¾H×\¿:;—ùä=T»$Ῠպ¾xãؾP[¿Æ®Y¿ïZ¾ñ"²¾'çˆ>AG>Ċn¿xjå>¹A"¿T4>ž‹>ëS¾z¨"¾¯«V¿Rc¾11龿òîºú#$>¾7:>;%=óU>ö6h¾ge¾ŽŒ>o¬5?µÔ¡>°+¥¾cÙ=P*?ñ¦ù<1Î}>ê̗?>¶¾ç‡à>'2n¾ÊØ~=ìñ·=×Õ£>
ìV>`ë?¬º?Ìs?>ÀŸ?§ÜM¾PŽÖ>L-ô½Ýt½$©Ñ½f$Ó>ªG¿Â0Ð>´¾Ô¾N6¾sÅ°>ïR㽇¬.¿dmŽ½ÃQÕ¾Ï)¾ÊX¿U~7¿‹¦Þ¾;ÂÀ>f¥K¾VR¾Øæ#=-š¾'-¾^
á>ÿø>^û¾¸¬ó¾˜†>i£¥¾:
¾jMÚ=¾¹?jÕ½˜¾S+]>uÚ|¾ÞL0¿)6Ô><	½`J?"¢¾Ô Q>2 ƒ¾¿‹¾cÁ>€»¾>€¾ìŽ½>)bh>A<佘 <L¸f¾ÛÆ»>B²P¾—»t¾™â¿ŒBj>!½½É›ã¾Vô´>¦?¾¸þ±>¯öú=hç¾	¹V<w¤'>jgܾ×÷8¿ï·>oH?Ied?î?×%?À}3>"*•¾E¡Ý=…W¿Ý$ܾÙ¨=3Cæ>û
a=•Æj¾ž™™>Շ=sž'>ÒÎ>'Uˆ=7|>Ú¥ù=_ú¿ø£?¨é¾
=}¾õ`>e•ü¼#ÿª>‡è©¾S)ø<Q-¾†xX¾¼ƒ8>¦Ý;¾8>by¾¦·Ô¾¯庥n×>mð>Æ¾Aé?Øüì¾BÚ_¿ž3?ý•û¼Ç߶>UY†¼©S·>]Á)¾m˒>֘1>:Ù8¾;¿><ö°¼=sļTœ>uÙÄ=.%<ÚMs¾{Î#½WFݽ¢F¿,¾÷/>íý½ªn¬¾

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/5_agent_zero_shot_from_4_policy/no_attn_ent/model/data/7 <==
%ܹèM=‡hѼúkG½ÿ䄽äGR½aœ=äý"½&"5<i̧<½£½žü'Âæ¼î°(½m*Ó»•	}<«É¢º´7¾œfI=ù­<Z¿a=öj»A†B½Êóá¼Sô»`pË<p»¾ah+>úCè<¼A½¡F–<Æ
½íA꼪‡…½šúç=;£N=@À=ÉË=ØÏA½\|Ÿ½U#f=VMw¾P#|=;m3½@s0=ü༚)Sºc'¼ï±'=–$†<å8=+½›á–=Qt¼kÏ
¾jÈN½DÔ<@[<"ÝQ½émI>#}õ;lŠ»R‹¾3Ü<Øü‹½À|k½h—½^.½"o;¢0¼‰x»Õ©3>±dš=N¿¼Ýr-=ˆ€¼¥"D=$f;FԚ¼NðS½Òub=f|g=tŽ£½'¼aے=Q°©¾YI°½"½^<;d>òÍ(½¿Žæ<y('½=¬5=>U<[Ì>cí?=õ÷®=ÐA½,Ó>¾Nî;ÿé=°.+½j³5¾¨r'=Òáí¼õ(J½òª<'l™¼ß½PS"¼Ès¾$öÌ=3踽_®<Ò2ð¼»	ö¼ý5½Ý¾½Ê*—¼$à=°]|½Ð"T¾Eƒç½§Ù=Ÿ¸:>ëʽ"[&½û
½VÃn½5ø>J±
:çÂ<ng_¾¹‰†<p³^> ¶<…#Û»Är=¡S­½sŽ>K¡==vW½ÁA=õ1¼ÊÀ=B;=š}½É3û»›šØº…¾gºË¦¦<A½&§Ÿ¼ög=ŒùÅ=›S±<,}Ø=n—¨¼O"í<éL(½ÂÖ½ñ`[<̪ÿ<¤O¼˜="Q<lÖ¼Qæ>µø&=È£ºÛµD½šMa>¶ÎM½OÏÆ»¾(k½úd =‡½?="ە=S½ûÑ">'øsºIˆ=‡«¾]3Ò=Å£H½œë
=t¤E=~«Ù<§'<½ð=NO9<pæ(=q#3½fK¡=Ê*P½Ü¸¾",¥¼{M"=µÿ1½Š,¡<+q\>€å½"¤=êŠ=Ã`Š>GÞ»B°:¾âæ¼8Më¼ËG¬½Zg•<œc=_äÿ·ÊZ±<|&½Ó"Ê=Îs½´v¤<ˆÒ¼¾Â½.¼Øº¥=m©¼àñJ½ÆÓ>Ljâ¼Ùüi¾ûq{½'<=¡Ã½ì1>ƒ¦ð½³W
½js=*oÁ<•0';˜A;nu꽊->`¬<¾6¡½.™½ßåÃ<C@­=Mo‰<~½çÝ=y¾bXɼ¦.ö=Ó»=
5Ý<û½Ë-ù½'ã+¼

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_3_policy/attn_ent/model/data/3 <==
¬‡¿HW¿uÌ<¿×WÇ>ED?ȧv¿M;ÀfŒ1¿Ô)¿/ÄE?7s"¿ö;?0?\‰×¿|*R¿&J£¿÷Ç?¹2»¿ô<î>G®¿ùi†>Ôý?CgÀ;¿Ji(À󕉿´ˆ¾¨qµ>øº¶¿×þÀj¯¿¸¯¿

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_3_policy/no_attn_ent/model/data/0 <==
Xºå<ké´;bÜ<!ž»L+A¼7ÿ<Ù¸á<w^N:¨/ó;ŠA¼W\<0T;<|*»úѹ;—껧Ú3»~æq:*³<ࡗ»±(2½€ËÙ;]n#¼-(Ÿ:F±X¼Ž
½7æ"<¬•ãº¯'¼'=¯<¼–Š<,÷Ö;´

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_4_policy/attn_ent/model/data/3 <==
ðß½÷>M#À°ŠV>"¿ÎMÚ>.áq¿²/ï¿÷bH¾Ä4Àäü¿we_¿¸%¿=Æ¾ìb¿½ÓÐ>ï-"¿êlÀ#ñ'¾)õe?Ӟ-¿¿­(ÀÐژ¿áGê>²׾)Ö?5m"=OïV¿×©´>\ô>£¹>BÌ?

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_4_policy/no_attn_ent/model/data/1 <==
'Ç8½2D¾¾ã(¾ª"Ÿ>Žº½@
–>Ivp¿^‰¼>'•Ë¾5rY½	¤¿!Ñ&½±a?´8\?ª×>Àä¬>Z>çK9>Ouu?|‹â¾ã¥œ>N¡|½µ>Ðoœ=1f‡>³V?q¼q>룰>‰ê'=æ`>†p¤?ø7=¾×¹½,gï>%kô>2,Ÿ=ä9E¿|"¾Ñ>
¾ó}½†R?>ô'‹>Qu¾Ÿš¿Íu>¿äþ¾ÃŒ,:Àº}>ÞÀÿ=;n=Éíe>‰ÛľoJ¾eÚw¾ÿ¢¿ÕaX>‰†¾°œ=ϏX=;Y½Îо§.?Ž3¾}NË>w+¾ë%C>IÐ=ty8?Ð =6@A?-Ö3½7$¾˜:?¬ßí>²gŒ¾ö >ë}¬¾ʱ½©œ'¾\y•=N$Ð>邿>Kgø>ë'Ï>P㌽Çôe¿ÂkÅ>â–ľ!§>ub>[Y¿‰1>¯âö>Ä4i?ÜÝ>;8¾œH¿O£>
¸¾Íjœ=Š×<ƒ>¢›?Cʅ¾°æê=¾‹>‰:?Xà ½€Ï(>Ñ¿¾n	>ÿî§=Ç(5=u¡7¿ûj¼¾…r¿Z¨=ôÍ>ʵ¾hÏݾãŸÕ>4ö›½Ú>?V¼€­(>pB¢<}yO¿B0b¿ƒËö¾ˆ6¿•Cà<P=ø°¶½A©s?*<s½²–>Ć>0c½J"оÕz'>
ŒÓ>"ÿÊ>¸Ã…¾wG<?…j>CS?Ã>m/U¾ç2O?®q¾Ë:?o9Ã>×bÀ>c8€¿äÒ?_oÔ=kó[¾…3"?îm>Ò´Ç=÷ò¾ð"ª¾Ê™è;´Ê¿ú9¾Úo
¾9\
¿"W
?Jü`?z=¿>e=@]¾Ï뫽+¬©=ðð¾'%?_Èo¾	oˆ>Rk/½$À7?¡ìE<"èƒ?^…¾Â•<Q n>ÄÇ«>,ñI½Úî¾Í]Pb¾ ´ˆ>4v¡»

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_4_policy/no_attn_ent/model/data/2 <==
ej¾É\#¼1"˾6ͼ1>¾H×\¿:;—ùä=T»$Ῠպ¾xãؾP[¿Æ®Y¿ïZ¾ñ"²¾'çˆ>AG>Ċn¿xjå>¹A"¿T4>ž‹>ëS¾z¨"¾¯«V¿Rc¾11龿òîºú#$>¾7:>;%=óU>ö6h¾ge¾ŽŒ>o¬5?µÔ¡>°+¥¾cÙ=P*?ñ¦ù<1Î}>ê̗?>¶¾ç‡à>'2n¾ÊØ~=ìñ·=×Õ£>
ìV>`ë?¬º?Ìs?>ÀŸ?§ÜM¾PŽÖ>L-ô½Ýt½$©Ñ½f$Ó>ªG¿Â0Ð>´¾Ô¾N6¾sÅ°>ïR㽇¬.¿dmŽ½ÃQÕ¾Ï)¾ÊX¿U~7¿‹¦Þ¾;ÂÀ>f¥K¾VR¾Øæ#=-š¾'-¾^
á>ÿø>^û¾¸¬ó¾˜†>i£¥¾:
¾jMÚ=¾¹?jÕ½˜¾S+]>uÚ|¾ÞL0¿)6Ô><	½`J?"¢¾Ô Q>2 ƒ¾¿‹¾cÁ>€»¾>€¾ìŽ½>)bh>A<佘 <L¸f¾ÛÆ»>B²P¾—»t¾™â¿ŒBj>!½½É›ã¾Vô´>¦?¾¸þ±>¯öú=hç¾	¹V<w¤'>jgܾ×÷8¿ï·>oH?Ied?î?×%?À}3>"*•¾E¡Ý=…W¿Ý$ܾÙ¨=3Cæ>û
a=•Æj¾ž™™>Շ=sž'>ÒÎ>'Uˆ=7|>Ú¥ù=_ú¿ø£?¨é¾
=}¾õ`>e•ü¼#ÿª>‡è©¾S)ø<Q-¾†xX¾¼ƒ8>¦Ý;¾8>by¾¦·Ô¾¯庥n×>mð>Æ¾Aé?Øüì¾BÚ_¿ž3?ý•û¼Ç߶>UY†¼©S·>]Á)¾m˒>֘1>:Ù8¾;¿><ö°¼=sļTœ>uÙÄ=.%<ÚMs¾{Î#½WFݽ¢F¿,¾÷/>íý½ªn¬¾

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_4_policy/no_attn_ent/model/data/7 <==
%ܹèM=‡hѼúkG½ÿ䄽äGR½aœ=äý"½&"5<i̧<½£½žü'Âæ¼î°(½m*Ó»•	}<«É¢º´7¾œfI=ù­<Z¿a=öj»A†B½Êóá¼Sô»`pË<p»¾ah+>úCè<¼A½¡F–<Æ
½íA꼪‡…½šúç=;£N=@À=ÉË=ØÏA½\|Ÿ½U#f=VMw¾P#|=;m3½@s0=ü༚)Sºc'¼ï±'=–$†<å8=+½›á–=Qt¼kÏ
¾jÈN½DÔ<@[<"ÝQ½émI>#}õ;lŠ»R‹¾3Ü<Øü‹½À|k½h—½^.½"o;¢0¼‰x»Õ©3>±dš=N¿¼Ýr-=ˆ€¼¥"D=$f;FԚ¼NðS½Òub=f|g=tŽ£½'¼aے=Q°©¾YI°½"½^<;d>òÍ(½¿Žæ<y('½=¬5=>U<[Ì>cí?=õ÷®=ÐA½,Ó>¾Nî;ÿé=°.+½j³5¾¨r'=Òáí¼õ(J½òª<'l™¼ß½PS"¼Ès¾$öÌ=3踽_®<Ò2ð¼»	ö¼ý5½Ý¾½Ê*—¼$à=°]|½Ð"T¾Eƒç½§Ù=Ÿ¸:>ëʽ"[&½û
½VÃn½5ø>J±
:çÂ<ng_¾¹‰†<p³^> ¶<…#Û»Är=¡S­½sŽ>K¡==vW½ÁA=õ1¼ÊÀ=B;=š}½É3û»›šØº…¾gºË¦¦<A½&§Ÿ¼ög=ŒùÅ=›S±<,}Ø=n—¨¼O"í<éL(½ÂÖ½ñ`[<̪ÿ<¤O¼˜="Q<lÖ¼Qæ>µø&=È£ºÛµD½šMa>¶ÎM½OÏÆ»¾(k½úd =‡½?="ە=S½ûÑ">'øsºIˆ=‡«¾]3Ò=Å£H½œë
=t¤E=~«Ù<§'<½ð=NO9<pæ(=q#3½fK¡=Ê*P½Ü¸¾",¥¼{M"=µÿ1½Š,¡<+q\>€å½"¤=êŠ=Ã`Š>GÞ»B°:¾âæ¼8Më¼ËG¬½Zg•<œc=_äÿ·ÊZ±<|&½Ó"Ê=Îs½´v¤<ˆÒ¼¾Â½.¼Øº¥=m©¼àñJ½ÆÓ>Ljâ¼Ùüi¾ûq{½'<=¡Ã½ì1>ƒ¦ð½³W
½js=*oÁ<•0';˜A;nu꽊->`¬<¾6¡½.™½ßåÃ<C@­=Mo‰<~½çÝ=y¾bXɼ¦.ö=Ó»=
5Ý<û½Ë-ù½'ã+¼

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_5_policy/attn_ent/model/data/5 <==
}(ƒ½N S=eÆ	¾\ñ°¼óöÈ=Rå)<žÖ
>ƍ´=ݸ'>@'=RÁ<æÛ»Ö%<¼'€ç=9«¿=Ò«<Ɨä=áؼå4¾¿1ì»7<MÓp½íÄg½åWë½í:x½3­ô¼ʙ½§=Ø<™Í@½hR™½6²¾ømÏ<ÂÛ>m)¾¹5¼Ð(ó<»\x=
'þ½­'½O;ʽã€í»	>¸Öì==*Ý:û漓91< ô=¿M'=Z,g<úü¾èú¾w=1!"»!×ä¼YL­=!õ½ Æ»=´IɽI�51½©û²½}+Š<€Éƒ½`˜J<&÷î¹8¯ß=n{µ<qT>n´Ñ½ŠÈ"½» ÿ=dȽPÔK=Ú0Å=t#Æ=kÓ½bT¼äŒý½db´=&9:=ëNý<ùïÁ<>
ó¼øK½w2§½ˆA<&ñ/;óL½ˆ7>ã'=!½t½GR+=	¸Ð<[èŸ=±JƽuJ°¼¼"Z=ª§˜=ו†»¨¤½÷*ˆ=à	>÷0­½Õ™=Ýñ	¾[^Ö½<'<_¯\¾Qö·¼ãŸá;Æç_<¨±½Ð˜½hÓ=_™'<ز¾"TA;'[Ú¼qˆÊ½¥·¾¼Ö½ÇÖ>¶G½StÈ=F'=
•¼ÿƒ;†"<|:@=¸m=G`¹"òå<yÎ2;þÌÌ=%GZ<õ_F¾¨Òø=\½¹9½šüH:©]©=µÔ²½3ü²¼ßR"¼Û;½AÊ.<Ð+C=òT»¾¨½^±F½>Ï<!.C½O=>¿pA>د€=ُ²½cS¹¼$J½4T½'wJ¾"½W=­O'½@\g½"B‡="Z´<Þ°¼d̆=¥Mü½x!€½ˆÊ³½S¥Ô½(—=¶àõ½cB½š«¤=L!¾<Fԑ½û%¤½(q½é'> @¾:jǽƒøö½Qû½Á	î½·ú÷;­ª=Õv¿=­1g½´aO¾µK»2¾å=Òtl½"F>|8?=ZÅ=4ìS>
N¾¹ëÉ<Jj:;Úaê=*ì½ðõ'<!-Á;ÐI¯½Ð^>̪½õ ×<àä=ÉL½‡#>Þ2¿½²ÁÛ<‹œ,>ä/½ä/Û»A~=ñ;7ߥ½Á'Å=œ¥»æŽ»=à€=´Y=£l	½ï¥<ê4½ˆ¡<pè?¼wÛÐ<§f¾q^p½À"š½‹¶z½ˆ¼ñX¾û¾½q×~½GĽ¼Ê䫼Qæœ;Հ½»´µ½*œ´=&ˆõ=r?ô<Šd<%ÿ½¨¡p=BÓ½Pü
>5Þ¯½K§|½Šª˜:…¶
=­
¾

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_5_policy/no_attn_ent/model/data/0 <==
nä¼b^»;%ˆ<¬'üw†¼á¼îN<–¨<²€¯<&t<ÊH~;5SW¼j°•»éO½@ĽáØU='ð'<±Æâ¼<å<쇖½5R!<²n<?´:ż;O;	<¼¶'½}c½|\(¼b‹í»óHŽ9'·¼

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/6_agent_zero_shot_from_5_policy/no_attn_ent/model/data/3 <==
)uŽ>ôñ'>§Ú?>¸µá¾ã'Ä<neƒ¿*)>nnQ=)¾='ݾ7q>˺©½—qÛ¿ŸPF¿
 é>WKG¿w¡>¬
y¿zÚ¾²*L¿G¼¿õ)z¿…2ˆ>®ï®>2Ü>Â\¿Y-|¿.è¾¥->Û6™¿1>¿‹¿

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/7_agent_zero_shot_from_4_policy/attn_ent/model/data/3 <==
ðß½÷>M#À°ŠV>"¿ÎMÚ>.áq¿²/ï¿÷bH¾Ä4Àäü¿we_¿¸%¿=Æ¾ìb¿½ÓÐ>ï-"¿êlÀ#ñ'¾)õe?Ӟ-¿¿­(ÀÐژ¿áGê>²׾)Ö?5m"=OïV¿×©´>\ô>£¹>BÌ?

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/7_agent_zero_shot_from_4_policy/no_attn_ent/model/data/1 <==
'Ç8½2D¾¾ã(¾ª"Ÿ>Žº½@
–>Ivp¿^‰¼>'•Ë¾5rY½	¤¿!Ñ&½±a?´8\?ª×>Àä¬>Z>çK9>Ouu?|‹â¾ã¥œ>N¡|½µ>Ðoœ=1f‡>³V?q¼q>룰>‰ê'=æ`>†p¤?ø7=¾×¹½,gï>%kô>2,Ÿ=ä9E¿|"¾Ñ>
¾ó}½†R?>ô'‹>Qu¾Ÿš¿Íu>¿äþ¾ÃŒ,:Àº}>ÞÀÿ=;n=Éíe>‰ÛľoJ¾eÚw¾ÿ¢¿ÕaX>‰†¾°œ=ϏX=;Y½Îо§.?Ž3¾}NË>w+¾ë%C>IÐ=ty8?Ð =6@A?-Ö3½7$¾˜:?¬ßí>²gŒ¾ö >ë}¬¾ʱ½©œ'¾\y•=N$Ð>邿>Kgø>ë'Ï>P㌽Çôe¿ÂkÅ>â–ľ!§>ub>[Y¿‰1>¯âö>Ä4i?ÜÝ>;8¾œH¿O£>
¸¾Íjœ=Š×<ƒ>¢›?Cʅ¾°æê=¾‹>‰:?Xà ½€Ï(>Ñ¿¾n	>ÿî§=Ç(5=u¡7¿ûj¼¾…r¿Z¨=ôÍ>ʵ¾hÏݾãŸÕ>4ö›½Ú>?V¼€­(>pB¢<}yO¿B0b¿ƒËö¾ˆ6¿•Cà<P=ø°¶½A©s?*<s½²–>Ć>0c½J"оÕz'>
ŒÓ>"ÿÊ>¸Ã…¾wG<?…j>CS?Ã>m/U¾ç2O?®q¾Ë:?o9Ã>×bÀ>c8€¿äÒ?_oÔ=kó[¾…3"?îm>Ò´Ç=÷ò¾ð"ª¾Ê™è;´Ê¿ú9¾Úo
¾9\
¿"W
?Jü`?z=¿>e=@]¾Ï뫽+¬©=ðð¾'%?_Èo¾	oˆ>Rk/½$À7?¡ìE<"èƒ?^…¾Â•<Q n>ÄÇ«>,ñI½Úî¾Í]Pb¾ ´ˆ>4v¡»

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/7_agent_zero_shot_from_4_policy/no_attn_ent/model/data/2 <==
ej¾É\#¼1"˾6ͼ1>¾H×\¿:;—ùä=T»$Ῠպ¾xãؾP[¿Æ®Y¿ïZ¾ñ"²¾'çˆ>AG>Ċn¿xjå>¹A"¿T4>ž‹>ëS¾z¨"¾¯«V¿Rc¾11龿òîºú#$>¾7:>;%=óU>ö6h¾ge¾ŽŒ>o¬5?µÔ¡>°+¥¾cÙ=P*?ñ¦ù<1Î}>ê̗?>¶¾ç‡à>'2n¾ÊØ~=ìñ·=×Õ£>
ìV>`ë?¬º?Ìs?>ÀŸ?§ÜM¾PŽÖ>L-ô½Ýt½$©Ñ½f$Ó>ªG¿Â0Ð>´¾Ô¾N6¾sÅ°>ïR㽇¬.¿dmŽ½ÃQÕ¾Ï)¾ÊX¿U~7¿‹¦Þ¾;ÂÀ>f¥K¾VR¾Øæ#=-š¾'-¾^
á>ÿø>^û¾¸¬ó¾˜†>i£¥¾:
¾jMÚ=¾¹?jÕ½˜¾S+]>uÚ|¾ÞL0¿)6Ô><	½`J?"¢¾Ô Q>2 ƒ¾¿‹¾cÁ>€»¾>€¾ìŽ½>)bh>A<佘 <L¸f¾ÛÆ»>B²P¾—»t¾™â¿ŒBj>!½½É›ã¾Vô´>¦?¾¸þ±>¯öú=hç¾	¹V<w¤'>jgܾ×÷8¿ï·>oH?Ied?î?×%?À}3>"*•¾E¡Ý=…W¿Ý$ܾÙ¨=3Cæ>û
a=•Æj¾ž™™>Շ=sž'>ÒÎ>'Uˆ=7|>Ú¥ù=_ú¿ø£?¨é¾
=}¾õ`>e•ü¼#ÿª>‡è©¾S)ø<Q-¾†xX¾¼ƒ8>¦Ý;¾8>by¾¦·Ô¾¯庥n×>mð>Æ¾Aé?Øüì¾BÚ_¿ž3?ý•û¼Ç߶>UY†¼©S·>]Á)¾m˒>֘1>:Ù8¾;¿><ö°¼=sļTœ>uÙÄ=.%<ÚMs¾{Î#½WFݽ¢F¿,¾÷/>íý½ªn¬¾

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/7_agent_zero_shot_from_4_policy/no_attn_ent/model/data/7 <==
%ܹèM=‡hѼúkG½ÿ䄽äGR½aœ=äý"½&"5<i̧<½£½žü'Âæ¼î°(½m*Ó»•	}<«É¢º´7¾œfI=ù­<Z¿a=öj»A†B½Êóá¼Sô»`pË<p»¾ah+>úCè<¼A½¡F–<Æ
½íA꼪‡…½šúç=;£N=@À=ÉË=ØÏA½\|Ÿ½U#f=VMw¾P#|=;m3½@s0=ü༚)Sºc'¼ï±'=–$†<å8=+½›á–=Qt¼kÏ
¾jÈN½DÔ<@[<"ÝQ½émI>#}õ;lŠ»R‹¾3Ü<Øü‹½À|k½h—½^.½"o;¢0¼‰x»Õ©3>±dš=N¿¼Ýr-=ˆ€¼¥"D=$f;FԚ¼NðS½Òub=f|g=tŽ£½'¼aے=Q°©¾YI°½"½^<;d>òÍ(½¿Žæ<y('½=¬5=>U<[Ì>cí?=õ÷®=ÐA½,Ó>¾Nî;ÿé=°.+½j³5¾¨r'=Òáí¼õ(J½òª<'l™¼ß½PS"¼Ès¾$öÌ=3踽_®<Ò2ð¼»	ö¼ý5½Ý¾½Ê*—¼$à=°]|½Ð"T¾Eƒç½§Ù=Ÿ¸:>ëʽ"[&½û
½VÃn½5ø>J±
:çÂ<ng_¾¹‰†<p³^> ¶<…#Û»Är=¡S­½sŽ>K¡==vW½ÁA=õ1¼ÊÀ=B;=š}½É3û»›šØº…¾gºË¦¦<A½&§Ÿ¼ög=ŒùÅ=›S±<,}Ø=n—¨¼O"í<éL(½ÂÖ½ñ`[<̪ÿ<¤O¼˜="Q<lÖ¼Qæ>µø&=È£ºÛµD½šMa>¶ÎM½OÏÆ»¾(k½úd =‡½?="ە=S½ûÑ">'øsºIˆ=‡«¾]3Ò=Å£H½œë
=t¤E=~«Ù<§'<½ð=NO9<pæ(=q#3½fK¡=Ê*P½Ü¸¾",¥¼{M"=µÿ1½Š,¡<+q\>€å½"¤=êŠ=Ã`Š>GÞ»B°:¾âæ¼8Më¼ËG¬½Zg•<œc=_äÿ·ÊZ±<|&½Ó"Ê=Îs½´v¤<ˆÒ¼¾Â½.¼Øº¥=m©¼àñJ½ÆÓ>Ljâ¼Ùüi¾ûq{½'<=¡Ã½ì1>ƒ¦ð½³W
½js=*oÁ<•0';˜A;nu꽊->`¬<¾6¡½.™½ßåÃ<C@­=Mo‰<~½çÝ=y¾bXɼ¦.ö=Ó»=
5Ý<û½Ë-ù½'ã+¼

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/7_agent_zero_shot_from_5_policy/attn_ent/model/data/5 <==
}(ƒ½N S=eÆ	¾\ñ°¼óöÈ=Rå)<žÖ
>ƍ´=ݸ'>@'=RÁ<æÛ»Ö%<¼'€ç=9«¿=Ò«<Ɨä=áؼå4¾¿1ì»7<MÓp½íÄg½åWë½í:x½3­ô¼ʙ½§=Ø<™Í@½hR™½6²¾ømÏ<ÂÛ>m)¾¹5¼Ð(ó<»\x=
'þ½­'½O;ʽã€í»	>¸Öì==*Ý:û漓91< ô=¿M'=Z,g<úü¾èú¾w=1!"»!×ä¼YL­=!õ½ Æ»=´IɽI�51½©û²½}+Š<€Éƒ½`˜J<&÷î¹8¯ß=n{µ<qT>n´Ñ½ŠÈ"½» ÿ=dȽPÔK=Ú0Å=t#Æ=kÓ½bT¼äŒý½db´=&9:=ëNý<ùïÁ<>
ó¼øK½w2§½ˆA<&ñ/;óL½ˆ7>ã'=!½t½GR+=	¸Ð<[èŸ=±JƽuJ°¼¼"Z=ª§˜=ו†»¨¤½÷*ˆ=à	>÷0­½Õ™=Ýñ	¾[^Ö½<'<_¯\¾Qö·¼ãŸá;Æç_<¨±½Ð˜½hÓ=_™'<ز¾"TA;'[Ú¼qˆÊ½¥·¾¼Ö½ÇÖ>¶G½StÈ=F'=
•¼ÿƒ;†"<|:@=¸m=G`¹"òå<yÎ2;þÌÌ=%GZ<õ_F¾¨Òø=\½¹9½šüH:©]©=µÔ²½3ü²¼ßR"¼Û;½AÊ.<Ð+C=òT»¾¨½^±F½>Ï<!.C½O=>¿pA>د€=ُ²½cS¹¼$J½4T½'wJ¾"½W=­O'½@\g½"B‡="Z´<Þ°¼d̆=¥Mü½x!€½ˆÊ³½S¥Ô½(—=¶àõ½cB½š«¤=L!¾<Fԑ½û%¤½(q½é'> @¾:jǽƒøö½Qû½Á	î½·ú÷;­ª=Õv¿=­1g½´aO¾µK»2¾å=Òtl½"F>|8?=ZÅ=4ìS>
N¾¹ëÉ<Jj:;Úaê=*ì½ðõ'<!-Á;ÐI¯½Ð^>̪½õ ×<àä=ÉL½‡#>Þ2¿½²ÁÛ<‹œ,>ä/½ä/Û»A~=ñ;7ߥ½Á'Å=œ¥»æŽ»=à€=´Y=£l	½ï¥<ê4½ˆ¡<pè?¼wÛÐ<§f¾q^p½À"š½‹¶z½ˆ¼ñX¾û¾½q×~½GĽ¼Ê䫼Qæœ;Հ½»´µ½*œ´=&ˆõ=r?ô<Šd<%ÿ½¨¡p=BÓ½Pü
>5Þ¯½K§|½Šª˜:…¶
=­
¾

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/7_agent_zero_shot_from_5_policy/no_attn_ent/model/data/0 <==
nä¼b^»;%ˆ<¬'üw†¼á¼îN<–¨<²€¯<&t<ÊH~;5SW¼j°•»éO½@ĽáØU='ð'<±Æâ¼<å<쇖½5R!<²n<?´:ż;O;	<¼¶'½}c½|\(¼b‹í»óHŽ9'·¼

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/7_agent_zero_shot_from_5_policy/no_attn_ent/model/data/3 <==
)uŽ>ôñ'>§Ú?>¸µá¾ã'Ä<neƒ¿*)>nnQ=)¾='ݾ7q>˺©½—qÛ¿ŸPF¿
 é>WKG¿w¡>¬
y¿zÚ¾²*L¿G¼¿õ)z¿…2ˆ>®ï®>2Ü>Â\¿Y-|¿.è¾¥->Û6™¿1>¿‹¿

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/8_agent_zero_shot_larger_env_from_5_policy/attn_ent/model/data/5 <==
}(ƒ½N S=eÆ	¾\ñ°¼óöÈ=Rå)<žÖ
>ƍ´=ݸ'>@'=RÁ<æÛ»Ö%<¼'€ç=9«¿=Ò«<Ɨä=áؼå4¾¿1ì»7<MÓp½íÄg½åWë½í:x½3­ô¼ʙ½§=Ø<™Í@½hR™½6²¾ømÏ<ÂÛ>m)¾¹5¼Ð(ó<»\x=
'þ½­'½O;ʽã€í»	>¸Öì==*Ý:û漓91< ô=¿M'=Z,g<úü¾èú¾w=1!"»!×ä¼YL­=!õ½ Æ»=´IɽI�51½©û²½}+Š<€Éƒ½`˜J<&÷î¹8¯ß=n{µ<qT>n´Ñ½ŠÈ"½» ÿ=dȽPÔK=Ú0Å=t#Æ=kÓ½bT¼äŒý½db´=&9:=ëNý<ùïÁ<>
ó¼øK½w2§½ˆA<&ñ/;óL½ˆ7>ã'=!½t½GR+=	¸Ð<[èŸ=±JƽuJ°¼¼"Z=ª§˜=ו†»¨¤½÷*ˆ=à	>÷0­½Õ™=Ýñ	¾[^Ö½<'<_¯\¾Qö·¼ãŸá;Æç_<¨±½Ð˜½hÓ=_™'<ز¾"TA;'[Ú¼qˆÊ½¥·¾¼Ö½ÇÖ>¶G½StÈ=F'=
•¼ÿƒ;†"<|:@=¸m=G`¹"òå<yÎ2;þÌÌ=%GZ<õ_F¾¨Òø=\½¹9½šüH:©]©=µÔ²½3ü²¼ßR"¼Û;½AÊ.<Ð+C=òT»¾¨½^±F½>Ï<!.C½O=>¿pA>د€=ُ²½cS¹¼$J½4T½'wJ¾"½W=­O'½@\g½"B‡="Z´<Þ°¼d̆=¥Mü½x!€½ˆÊ³½S¥Ô½(—=¶àõ½cB½š«¤=L!¾<Fԑ½û%¤½(q½é'> @¾:jǽƒøö½Qû½Á	î½·ú÷;­ª=Õv¿=­1g½´aO¾µK»2¾å=Òtl½"F>|8?=ZÅ=4ìS>
N¾¹ëÉ<Jj:;Úaê=*ì½ðõ'<!-Á;ÐI¯½Ð^>̪½õ ×<àä=ÉL½‡#>Þ2¿½²ÁÛ<‹œ,>ä/½ä/Û»A~=ñ;7ߥ½Á'Å=œ¥»æŽ»=à€=´Y=£l	½ï¥<ê4½ˆ¡<pè?¼wÛÐ<§f¾q^p½À"š½‹¶z½ˆ¼ñX¾û¾½q×~½GĽ¼Ê䫼Qæœ;Հ½»´µ½*œ´=&ˆõ=r?ô<Šd<%ÿ½¨¡p=BÓ½Pü
>5Þ¯½K§|½Šª˜:…¶
=­
¾

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/8_agent_zero_shot_larger_env_from_5_policy/no_attn_ent/model/data/0 <==
nä¼b^»;%ˆ<¬'üw†¼á¼îN<–¨<²€¯<&t<ÊH~;5SW¼j°•»éO½@ĽáØU='ð'<±Æâ¼<å<쇖½5R!<²n<?´:ż;O;	<¼¶'½}c½|\(¼b‹í»óHŽ9'·¼

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/8_agent_zero_shot_larger_env_from_5_policy/no_attn_ent/model/data/3 <==
)uŽ>ôñ'>§Ú?>¸µá¾ã'Ä<neƒ¿*)>nnQ=)¾='ݾ7q>˺©½—qÛ¿ŸPF¿
 é>WKG¿w¡>¬
y¿zÚ¾²*L¿G¼¿õ)z¿…2ˆ>®ï®>2Ü>Â\¿Y-|¿.è¾¥->Û6™¿1>¿‹¿

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/symm_kl_120/attn_ent/model120/data/2 <==
#ØQ=Õ!i?Ë$>1Ûí¾®'<<™I?¹¯7¾ËQü>Ñ¿+0R>辕r¿ŽÊ&>̤?Ÿèù¾y=ø½ï!?ŠŽ`>$‡S¾N‡¾ý¿¿½kEË>J_V¾R
ì>8r¼½uÏû>>">®É>c
>ÂAß¾ú?òòѾ8>ñº	¿rƒH>mh¿Gúœ¿Þââ½ÛIû¾Bf>–>Ùö\>숇¾…ˆ·¾CŠ'>€å?e•'¿N–þ½b}ľ6#?dµ?oJÏ>ìl¼òÁܾŠ³þ¾|<«Úú¾¶€‹>«ÔŽ¾eqÒ½¼/>é_=>µ4¿9+@¿â¬¢;;ŵ>Õ=n±ü¾;¡=ËÛ²¾û"¾¾.ó>jõ¥=¨"6¾ZÔn=îöm¾,î7?µ¨U¿þUß>‹ü=¨"ݾw2ƒ½ÓH"=q'Þ¾ Ï`>6>
= €¿Â¥®>0õ¡>Èg?K"k>üv>²Nµ>­J>©¨}¼l×>Uw>*»D>f[Ǿ›G6>>õ¿AÞv¿<°Ñ¼—¿š3j>ƾ"½ [œ=V9í<ž©.?™½;
?U&{?%©¿Q'>wæ¿–ßG=•Œk¾£ò>Â0¾‹O¤>Cb¾¡º{>ã
?/ƒ«¾%yÿ<~¾¾8[»¾©4˜¾ïo•½¦Y¦?°/?èµy>ÐB'>[š©¾gå¼]èü>s ¾j]½¼Œ˜>¬™Å='=¿Sº´¿nÅ	> Q#¾_4\¼"7>8"Ù½ÚB¦¾ -?Ö»¡>iå>å
>~G—>Þúí=íi¡¼÷—7¾ûk˜=¤,Ö>æ¢?­,>>¨½)u">˜ˆZ>›Ì?<©þ>Ýw?Lv¿§U…½MƇ¾(ûÿ¾© ?Z)+¿R4™?¥Š¶¾v´?"<.>™W¦½]I/¿<®¾*
ú¾~¶I½<®>úªW½RqŽ?X'×¾t¹Ï<@d‹=q‡>R W>

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/symm_kl_120/attn_ent/model120/data/3 <==
®N…¿¡EM¿n6¿§ÌÀ>j¢B?/n¿<xÀ?¢+¿2Ê!¿Ì<?Jï¿üÐ?y^ý>dÍ¿©HE¿Y[¿=?+µ¿æ>ΰ£¿VéH>í™?1wÀ"Ä9¿"ÀHŽ'¿©`w¾*f›>j…¯¿\ÀSx§¿®Aª¿

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/symm_kl_30/no_attn_ent/model30/data/0 <==
Șµ<Y×b¼ezª¹Àÿ8»xݼëèc;qJÈ<I¼>‰#<GU»}œ";ôré»°<sm<¥n<_;º[<ŸpÐ<5;ã;''Š:îþ;²Sš¼Ïž×¹ÍÚr¼`\":ש;2ކ¼¬Ü™¼k<ñ¼ìœ¼â&½

==> AAMAS-2025-Formatting-Instructions-CCBY/fig/symm_kl_30/no_attn_ent/model30/data/2 <==
,Š<ӏ?ßMÅ>Wn˾Õ8	>
Ò?¸ÎE¾Û»ã>¿±œ¾D©=…Bä¾Å
î¾y×è=x! >/>㾨¹='µ—<E#ë>Îúw>,Bƽ»V'¾â|…;Ùà™>´Ú;ˆÚ¶>É·¦½ëî'>ˆÿ';¨ò­<ÑÉ=>Ökþ¾ê¹?Tª"¾áŠ>Îß¿-¸µ=Þ¾ŒdM¿íÖö½¯|˜¾8µR>DdF>,Y>&­I¾qޙ¾8Y³>Ô
ƒ>Öv¿ê ¾bn¾ö°Ñ>xw?ÿJ'> n+>"L¾1Tç¾Ùˆ¾Ø¾øèÞ¾&&«>­¤}¾é>Ö¼]Dý=܋…=•r¿oq¿/~Á=ǵ>]q¾Rjž¾°8">¡¾B)¾U°Ã>°mG¾‡Ü=Ÿe>dìs¾=«Ê>t6,¿f!>ڞ>ïhʾ¿ƒ¾4pê¼m|–¾áu>×Ò«½40¿©,‡>C+>ÕÔ?¶²Ü=¡ ó=í±Ô>vƒŸ=¶H>\-x>«Þ@>É>޽˜A¾˜ˆ½¸×¾îž¿Qˋ½½A©¾§'^>C'¾'§ó½ú
¾úD´½ÔÖ>ݹk½XÒ>̌8?ÞþAö>FS¿¿r	>öÖ¨¾Tò?+¾	
->RÈ ¾½5G>EwÙ>:D±¾N€<Œ´¾³u»¾¤Ac¾Sr¾€Z?ëó'>…='¼/²>sÜr¾IZ+¼éÊ>•x=¾I"^¾Ê>?X½Íø¿X\{¿Ê">A'»VÍc=žûù=-H&¾:ž°¾ÛÎ>Ò>q7ã>a¹>òº>Cc?Cæ0>pÔ\¾X''½¢è°>6û¥>ÛË>¾R½‹Ôæ= £>FÁØ>ãEÓ>Ï >9Ú羈'²¾'Ž¥¾u]þ[¿>54¿¯Ð7?d#…¾õŸÕ>e =Q
Ð;»$e¾2	›¾ÙU‡¾QÜZ>—£Ÿ=µƒª½v\=?YIÓ¾`µ¾Í¢=c¿{>^—½=
